Investigation of the stability in the performance of triple GEM detectors for High Energy Physics experiments

Gas Electron Multiplier (GEM) is one of the mostly used gaseous detectors in the High Energy Physics (HEP) experiments. GEMs are widely used as tracking devices due to their high-rate handling capability and good position resolution. An initiative is taken to study the stability in performance of the GEM chamber prototypes in the laboratory using external radiation for different Argon based gas mixtures. The effect of ambient parameters on the gain and energy resolution are studied. Very recently some behavioural changes in the performance of a SM GEM chamber is observed. The details of the experimental setup, methodology and results are reported here.

==> makefile.tex <==
# $Id: makefile 193 2020-11-23 11:15:37Z rishi $

file=elsdoc


all: pdf out 
	make pdf
	make pdf

out:
	if  [ -f $(file).out ] ; then cp $(file).out tmp.out; fi ;
	sed 's/BOOKMARK/dtxmark/g;' tmp.out > x.out; mv x.out tmp.out ;

pdf:
	pdflatex $(file).tex

index:
	makeindex -s gind.ist -o $(file).ind $(file).idx 

changes:
	makeindex -s gglo.ist -o $(file).gls $(file).glo

xview:
#	xpdf -z 200 $(file).pdf &>/dev/null
	open -a 'Skim.app' $(file).pdf 

view:
	open -a 'Adobe Reader.app' $(file).pdf

ins:
	latex $(file).ins 

diff:
	diff $(file).sty ../$(file).sty |less

copy:
	cp $(file).sty ../






